The ELM Survey South. II. Two dozen new low mass white dwarf binaries

We present the results from our ongoing spectroscopic survey targeting low mass white dwarf binaries, focusing on the southern sky. We used a Gaia DR2 and eDR3 based selection and identified 28 new binaries, including 19 new extremely low mass white dwarfs, one short period, likely eclipsing, DABZ, and two potential LISA binaries. We present orbital and atmospheric parameters for each new binary based on our spectroscopic follow-up. Four of our new binaries show periodic photometric variability in the TESS 2-minute cadence data, including one new eclipsing double-lined spectroscopic binary. Three others show periodic photometric variability in ZTF, including one new eclipsing binary. We provide estimates for the inclinations and scaled component radii for these ZTF variables, based on light curve modeling to our high-speed photometric follow-up observations. Our observations have increased the sample of ELM Survey binaries identified in the southern sky to 41, an increase of 64%. Future time domain surveys, such as BlackGEM and the Vera C. Rubin Observatory Legacy Survey of Space and Time, will efficiently identify the photometric variables in the southern sky and significantly increase the population of southern sky low mass white dwarf binaries, leading to a more complete all-sky population of these systems.

==> lcurve_table.tex <==
\begin{table}
\center
  \renewcommand{\arraystretch}{1.5}
  \addtolength{\tabcolsep}{2pt}
    % \vspace*{1cm}
	\begin{tabular}{l c c}
    \hline
    \hline
    {} & \multicolumn{1}{C}{\rm J0221$+$1710} & \multicolumn{1}{C}{\rm J2049$+$3351}\\
    \hline
    {$q$} & \nodata & $0.39\pm0.2$ \\
    {$i~({\rm ^\circ})$} & $89.0\pm0.2$ & $74^{+3}_{-2}$ \\
    {$R_1/a$} & $0.045\pm0.001$ & $0.31\pm0.05$ \\
    {$R_2/a$} & $0.020\pm0.001$ & $0.06^{+0.03}_{-0.02}$ \\
    {$T_{\rm eff,1}~({\rm K})$} & ($13400\pm180$) & $23200^{+4900}_{-4300}$ \\
    {$T_{\rm eff,2}~({\rm K})$} & $\lesssim6400$ & $35400^{+9700}_{-8600}$ \\
    \hline
    \hline
	\end{tabular}
    \caption{System parameters for J0211$+$1710 and J2049$+$3351 obtained through fitting photometric variability with \textsc{lcurve} as described in the text.}
    \label{table:lcurve_table}
\end{table}
